Carbon and Oxygen in Nearby Stars: Keys to Protoplanetary Disk Chemistry

We present carbon and oxygen abundances for 941 FGK stars-the largest such catalog to date. We find that planet-bearing systems are enriched in these elements. We self-consistently measure C/O, which is thought to play a key role in planet formation. We identify 46 stars with C/O \geq 1.00 as potential hosts of carbon-dominated exoplanets. We measure a downward trend in [O/Fe] versus [Fe/H] and find distinct trends in the thin and thick disks, supporting the work of Bensby et al. Finally, we measure sub-solar C/O = 0.40+0.11 - 0.07, for WASP-12, a surprising result as this star is host to a transiting hot Jupiter whose dayside atmosphere was recently reported to have C/O \geq 1 by Madhusudhan et al. Our measurements are based on 15,000 high signal-to-noise spectra taken with the Keck 1 telescope as part of the California Planet Search. We derive abundances from the [O I] and C I absorption lines at {\lambda} = 6300 and 6587 {\AA} using the SME spectral synthesizer.

==> xonfe.tex <==

[C/Fe] & thick & -0.550 $\pm$ 0.074 & 0.074 $\pm$ 0.035 & 2.19 \\

[C/Fe] & thin & -0.318 $\pm$ 0.019 & 0.021 $\pm$ 0.004 & 2.52 \\

[O/Fe] & thick & -0.475 $\pm$ 0.081 & 0.260 $\pm$ 0.047 & 2.41 \\

[O/Fe] & thin & -0.642 $\pm$ 0.017 & 0.067 $\pm$ 0.004 & 1.66 \\

